Variational Inference with Parameter Learning Applied to Vehicle Trajectory Estimation

We present parameter learning in a Gaussian variational inference setting using only noisy measurements (i.e., no groundtruth). This is demonstrated in the context of vehicle trajectory estimation, although the method we propose is general. The paper extends the Exactly Sparse Gaussian Variational Inference (ESGVI) framework, which has previously been used for large-scale nonlinear batch state estimation. Our contribution is to additionally learn parameters of our system models (which may be difficult to choose in practice) within the ESGVI framework. In this paper, we learn the covariances for the motion and sensor models used within vehicle trajectory estimation. Specifically, we learn the parameters of a white-noise-on-acceleration motion model and the parameters of an Inverse-Wishart prior over measurement covariances for our sensor model. We demonstrate our technique using a 36~km dataset consisting of a car using lidar to localize against a high-definition map; we learn the parameters on a training section of the data and then show that we achieve high-quality state estimates on a test section, even in the presence of outliers. Lastly, we show that our framework can be used to solve pose graph optimization even with many false loop closures.

==> notation.tex <==

\section{General Notation}

\begin{center}
\begin{tabular}{rl}
$a$ & Symbols in this font are real scalars.\\
$\mbf{a}$ & Symbols in this font are real column vectors. \\
$\mbf{A}$ & Symbols in this font are real matrices. \\
$\mathcal{A}$ & Symbols in this font are sigma-points used in the Unscented Transformation, except $\mathcal{N}$, $\mathcal{F}$, and $\mathcal{O}$, \\ &  which have special meanings. \\
$p(\mbf{a})$ & The probability density of $\mbf{a}$. \\
 $p( \mbf{a} |
\mbf{b} )$ & The probability density of $\mbf{a}$ given
$\mbf{b}$. \\
$\sim\mathcal{N}(\mbf{a}, \mbf{B})$ & Normally distributed with
mean
$\mbf{a}$ and covariance $\mbf{B}$. \\
$\mathcal{O}$ & Observability matrix. \\
$(\cdot)_k$ & The value of a quantity at timestep $k$. \\
$(\cdot)_{k_1:k_2}$ & The set of values of a quantity from timestep $k_1$ to timestep $k_2$, inclusive.\\
%$\mbf{a}^{(m)}$ & Superscript $(m)$ is the index of a sample drawn from a density. \\
$\Vec{\bcf}_a$ & A vectrix representing a reference frame in three dimensions. \\
$ \Vec{a}$ & A vector quantity in three dimensions. \\
$(\cdot)^\times$ & The cross-product operator which produces a
skew-symmetrix matrix from a column. \\
$\mbf{1}$ & The identity matrix. \\
$\mbf{0}$ & The zero matrix. \\
\end{tabular}
\end{center}

\newpage
\section{Specific Notation and Background}
\label{sec:notation}

\subsection{\em Exponential Map, Lie Bracket, and the Baker-Campbell-Hausdorff Formula}

The following definitions, identities, and approximations are useful for handling exponential maps of matrices.
\begin{eqnarray*}
e^\mbf{A}  & :=  & \sum_{n=0}^\infty \frac{1}{n!} \mbf{A}^n \qquad \mbox{(\em matrix exponential)} \\
& = & \mbf{1} + \mbf{A} + \frac{1}{2} \mbf{A} \mbf{A} + \frac{1}{6} \mbf{A}\mbf{A}\mbf{A} + \frac{1}{24} \mbf{A}\mbf{A}\mbf{A} \mbf{A} + \cdots \\
\log \mbf{A} & := & \sum_{n=1}^\infty \frac{(-1)^{n-1}}{n}\left( \mbf{A} - \mbf{1} \right)^n \qquad \mbox{(\em matrix logarithm)} \\
\log \left( e^\mbf{A} \right) & \equiv & \mbf{A}   \\
\frac{d}{dt} e^{\mbf{A}}  & \equiv & \int_0^1 e^{\alpha\mbf{A}} \, \frac{d\mbf{A}}{dt} \, e^{(1-\alpha)\mbf{A}} \, d\alpha  \qquad \mbox{(\em derivative of matrix exponential)} 
\end{eqnarray*}
\begin{gather*}
\left[ \mbf{A}, \mbf{B} \right]  :=  \mbf{A} \mbf{B} - \mbf{B} \mbf{A} \qquad \mbox{(\em Lie bracket)} \\
\left[ \mbf{A}, \mbf{B} \right] \equiv -\left[ \mbf{B}, \mbf{A} \right], \qquad \left[\mbf{A},\mbf{A}\right] \equiv \mbf{0} \\
\left[ \mbf{A}, \left[ \mbf{B}, \mbf{C} \right] \right]+ \left[ \mbf{C}, \left[ \mbf{A}, \mbf{B} \right] \right] + \left[ \mbf{B}, \left[ \mbf{C}, \mbf{A} \right] \right] \equiv \mbf{0} \qquad \mbox{(\em Jacobi identity)}
\end{gather*}
\begin{eqnarray*}
e^{\mbf{A}+\mbf{B}} & = & \lim_{\alpha\rightarrow\infty} \left( e^{\mbf{A}/\alpha} e^{\mbf{B}/\alpha} \right)^{\alpha} \qquad \mbox{(\em Lie product formula)} \\
\log\left( e^\mbf{A} e^\mbf{B} \right) & \equiv & \sum_{n=1}^\infty \frac{(-1)^{n-1}}{n} \sum_{\begin{scriptsize}\begin{array}{c} r_i+s_i>0, \\ 1\leq i \leq n\end{array}\end{scriptsize}} \frac{\left( \sum_{i=1}^n (r_i+s_i) \right)^{-1}}{\prod_{i=1}^n r_i ! s_i !} \left[ \mbf{A}^{r_1} \mbf{B}^{s_1}\mbf{A}^{r_2} \mbf{B}^{s_2} \cdots \mbf{A}^{r_n}\mbf{B}^{s_n} \right] \qquad \mbox{(\em BCH formula)} \\
& = & \mbf{A} + \mbf{B} + \frac{1}{2} \left[ \mbf{A}, \mbf{B} \right] + \frac{1}{12} \left[ \mbf{A}, \left[ \mbf{A}, \mbf{B} \right] \right] - \frac{1}{12} \left[ \mbf{B}, \left[ \mbf{A}, \mbf{B} \right] \right] - \frac{1}{24} \left[ \mbf{B}, \left[ \mbf{A}, \left[ \mbf{A}, \mbf{B} \right] \right] \right] \\
&  & \; - \; \frac{1}{720} \left( \left[ \left[ \left[ \left[ \mbf{A}, \mbf{B} \right] ,\mbf{B} \right], \mbf{B} \right], \mbf{B} \right] + \left[ \left[ \left[ \left[ \mbf{B}, \mbf{A} \right] ,\mbf{A} \right], \mbf{A} \right], \mbf{A} \right] \right) \; + \; \frac{1}{360} \left( \left[ \left[ \left[ \left[ \mbf{A}, \mbf{B} \right] ,\mbf{B} \right], \mbf{B} \right], \mbf{A} \right] + \left[ \left[ \left[ \left[ \mbf{B}, \mbf{A} \right] ,\mbf{A} \right], \mbf{A} \right], \mbf{B} \right] \right)\\
&  & \; + \; \frac{1}{120} \left( \left[ \left[ \left[ \left[ \mbf{A}, \mbf{B} \right] ,\mbf{A} \right], \mbf{B} \right], \mbf{A} \right] + \left[ \left[ \left[ \left[ \mbf{B}, \mbf{A} \right] ,\mbf{B} \right], \mbf{A} \right], \mbf{B} \right] \right) \; + \; \cdots \\
& \equiv & \mbf{A} + \mbf{B} \qquad \mbox{(if and only if $\mbf{A}$ and $\mbf{B}$ commute, i.e., $\mbf{A}\mbf{B}=\mbf{B}\mbf{A}$ or $[\mbf{A},\mbf{B}]=\mbf{0}$)}
\end{eqnarray*}
\begin{eqnarray*}
\left[ \mbf{A}^{r_1} \mbf{B}^{s_1}\mbf{A}^{r_2} \mbf{B}^{s_2} \cdots \mbf{A}^{r_n}\mbf{B}^{s_n} \right]  & := & \underbrace{\bigl[ \mbf{A}, \ldots \bigl[ \mbf{A},}_{r_1} \underbrace{\bigl[ \mbf{B}, \ldots, \bigl[ \mbf{B},}_{s_1} \ldots \underbrace{\bigl[ \mbf{A}, \ldots \bigl[ \mbf{A},}_{r_n} \underbrace{\bigl[ \mbf{B}, \ldots \bigl[ \mbf{B}, \mbf{B} \bigr] \ldots \bigr] }_{s_n} \bigr] \ldots \bigr] \ldots \bigr] \ldots \bigr] \bigr] \ldots \bigr] \\
& = & \mbf{0} \quad \mbox{(if $s_n > 1$ or  if $s_n=0$ and $r_n > 1$)}
\end{eqnarray*}
\begin{eqnarray*}
\log\left( e^\mbf{A} e^\mbf{B} \right) & \approx & \mbf{A} + \sum_{n=0}^\infty (-1)^n \frac{B_n}{n!} \underbrace{\bigl[ \mbf{A}, \bigl[ \mbf{A}, \ldots \bigl[ \mbf{A},}_{n} \mbf{B} \bigr] \ldots \bigr] \bigr] \qquad \mbox{(keeping all terms up to linear in $\mbf{B}$ \cite{klarsfeld89})} \\
\log\left( e^\mbf{A} e^\mbf{B} \right) & \approx & \mbf{B} + \sum_{n=0}^\infty \frac{B_n}{n!} \underbrace{\bigl[ \mbf{B}, \bigl[ \mbf{B}, \ldots \bigl[ \mbf{B},}_{n} \mbf{A} \bigr] \ldots \bigr] \bigr] \\
& & \qquad\qquad\qquad \mbox{(keeping all terms up to linear in $\mbf{A}$; hint: use $e^\mbf{A} e^\mbf{B} = \left( e^{-\mbf{B}}e^{-\mbf{A}} \right)^{-1}$ with previous)}
\end{eqnarray*}
\begin{gather*}
B_0 = 1, B_1 = -\frac{1}{2}, B_2 = \frac{1}{6}, B_3 = 0, B_4 = -\frac{1}{30}, B_5 = 0, \ldots \qquad \mbox{(\em Bernoulli numbers)}
\end{gather*}

\subsection{{\em SO(3)} Notation}

\noindent
The following definitions, identities, and approximations are useful for {\em SO(3)}.  Some can be found in \citet{hughes86}.
\begin{gather*}
\mbf{u}^\times = \bbm u_1 \\ u_2 \\ u_3 \ebm^\times := \bbm 0 & -u_3 & u_2 \\ u_3 & 0 & -u_1 \\ -u_2 & u_1 & 0 \ebm \\
\left( \alpha \mbf{u} + \beta \mbf{v} \right)^\times \equiv \alpha \mbf{u}^\times + \beta \mbf{v}^\times \\
\mbf{u}^{\times^T} \equiv -\mbf{u}^\times \\
\mbf{u}^\times \mbf{v} \equiv - \mbf{v}^\times \mbf{u}, \qquad \mbf{u}^\times \mbf{u} \equiv \mbf{0} \\
\left(\mbf{A} \mbf{u}\right)^\times \equiv \mbf{u}^\times \left( \mbox{tr}(\mbf{A}) \, \mbf{1} - \mbf{A} \right) - \mbf{A}^T \mbf{u}^\times \\
\mbf{u}^\times \mbf{v}^\times \equiv - (\mbf{u}^T\mbf{v})\, \mbf{1} + \mbf{v} \mbf{u}^T \\
\mbf{u}^\times \mbf{A} \, \mbf{v}^\times \equiv - \left(-\mbox{tr}(\mbf{v}\mbf{u}^T) \, \mbf{1} + \mbf{v}\mbf{u}^T \right)\left( -\mbox{tr}(\mbf{A}) \, \mbf{1} + \mbf{A}^T \right) + \mbox{tr}(\mbf{A}^T \mbf{v} \mbf{u}^T ) \, \mbf{1} - \mbf{A}^T \mbf{v} \mbf{u}^T \\
\mbf{u}^\times\mbf{v}^\times\mbf{u}^\times \equiv \mbf{u}^\times \mbf{u}^\times \mbf{v}^\times + \mbf{v}^\times \mbf{u}^\times \mbf{u}^\times + (\mbf{u}^T \mbf{u}) \, \mbf{v}^\times \\
\mbf{u}^\times \mbf{u}^\times \mbf{u}^\times \equiv -(\mbf{u}^T\mbf{u}) \, \mbf{u}^\times \\
\mbf{u}^\times\mbf{v}^\times\mbf{v}^\times- \mbf{v}^\times\mbf{v}^\times\mbf{u}^\times \equiv (\mbf{v}^\times\mbf{u}^\times\mbf{v})^\times \\
\left[ \mbf{u}^\times, \mbf{v}^\times \right]  \equiv \mbf{u}^\times\mbf{v}^\times - \mbf{v}^\times \mbf{u}^\times \equiv  \left( \mbf{u}^\times\mbf{v}\right)^\times, \qquad \underbrace{\bigl[ \mbf{u}^\times, \bigl[ \mbf{u}^\times, \ldots \bigl[ \mbf{u}^\times,}_{n} \mbf{v}^\times \bigr] \ldots \bigr] \bigr] \equiv \left( \left( \mbf{u}^\times \right)^n \mbf{v} \right)^\times \\
\mbs{\phi} := \phi \mbf{a} \\
\mbf{C} := \cos\phi \mbf{1} + (1-\cos\phi) \mbf{a}\mbf{a}^T - \sin\phi \mbf{a}^\times \equiv e^{-\mbs{\phi}^\times}  \equiv \sum_{n=0}^\infty(-1)^n \frac{1}{n!}\left(\mbs{\phi}^\times\right)^n  \approx \mbf{1} - \mbs{\phi}^\times  \\
\mbox{tr}(\mbf{C}) \equiv 2 \cos\phi + 1, \qquad \mbox{det} (\mbf{C}) \equiv 1 \\
\mbf{C} \mbf{a} \equiv \mbf{a}, \qquad \mbf{C} \mbf{a}^\times \equiv \mbf{a}^\times \mbf{C} \\ 
\mbf{C}^{-1} \equiv \mbf{C}^T \equiv \sum_{n=0}^\infty \frac{1}{n!}\left(\mbs{\phi}^\times\right)^n \approx \mbf{1} + \mbs{\phi}^\times\\ 
\mbf{C}^T \mbf{C} \equiv \mbf{1} \equiv \mbf{C} \mbf{C}^T \\ 
\left(\mbf{C} \mbf{u} \right)^\times \equiv \mbf{C} \mbf{u}^\times \mbf{C}^T, \qquad e^{(\mbf{C}\mbf{u})^\times}\equiv \mbf{C} e^{\mbf{u}^\times}  \mbf{C}^T \\
\mbf{S} := \int_0^1 \mbf{C}^\alpha \, d\alpha  \equiv \sum_{n=0}^\infty(-1)^n \frac{1}{(n+1)!}\left(\mbs{\phi}^\times\right)^n  \equiv \frac{\sin\phi}{\phi} \mbf{1} + \left( 1 - \frac{\sin\phi}{\phi} \right) \mbf{a}\mbf{a}^T - \frac{1-\cos\phi}{\phi} \mbf{a}^\times \approx \mbf{1}- \frac{1}{2} \mbs{\phi}^\times \\
\mbf{S}^{-1}  \equiv \sum_{n=0}^\infty(-1)^n \frac{B_n}{n!}\left(\mbs{\phi}^\times\right)^n \equiv \frac{\phi}{2}\cot\frac{\phi}{2}\mbf{1} + \left( 1 - \frac{\phi}{2}\cot\frac{\phi}{2}\right)\mbf{a}\mbf{a}^T + \frac{\phi}{2} \mbf{a}^\times  \approx \mbf{1} + \frac{1}{2}\mbs{\phi}^\times\\
\qquad\qquad\qquad \mbox{($B_n$ are Bernouilli numbers defined above; does not exist for $\phi=2\pi m$, $m\neq 0$; trigonometric version in \cite{hughes86})} \\
e^{-\left(\mbf{u} + \mbs{\phi}\right)^\times} \approx e^{-(\mbf{S} \mbf{u})^\times} \mbf{C}, \qquad \mbox{(correct to first order in $\mbf{u}$)} \\
\mbf{C} \equiv \mbf{1} - \mbs{\phi}^\times \mbf{S} \\
\frac{\partial \left( \mbf{C} \mbf{v} \right) }{\partial \mbs{\phi}} =  \left( \mbf{C} \mbf{v} \right)^\times \mbf{S}
\end{gather*}

\subsection{Quaternion Notation}

The following definitions, identities, and approximations are useful for quaternion representations of points and rotations.  Much of this notation can be found in \citet{barfoot_aa11}.
\begin{gather*}
\mbf{u}^\eqm := \frac{1}{2} \bbm \mbf{u}^\times & -\mbf{u} \\ \mbf{u}^T & 0 \ebm, \qquad \mbf{u}^\eqp := \frac{1}{2} \bbm -\mbf{u}^\times & -\mbf{u} \\ \mbf{u}^T & 0 \ebm \\
\left( \alpha \mbf{u} + \beta \mbf{v} \right)^\eqm \equiv \alpha \mbf{u}^\eqm + \beta \mbf{v}^\eqm,  \qquad \left( \alpha \mbf{u} + \beta \mbf{v} \right)^\eqp \equiv \alpha \mbf{u}^\eqp + \beta \mbf{v}^\eqp \\
\mbf{u}^{\eqm^T} \equiv -\mbf{u}^\eqm, \qquad \mbf{u}^{\eqp^T} \equiv -\mbf{u}^\eqp \\
\mbf{u}^\eqm \mbf{u}^\eqm = -\frac{1}{4} (\mbf{u}^T \mbf{u}) \, \mbf{1}, \qquad  \mbf{u}^\eqp \mbf{u}^\eqp = -\frac{1}{4} (\mbf{u}^T \mbf{u}) \, \mbf{1} \\
\left[ \mbf{u}^\eqm, \mbf{v}^\eqm \right] \equiv \mbf{u}^\eqm \mbf{v}^\eqm - \mbf{v}^\eqm \mbf{u}^\eqm \equiv \left( \mbf{u}^\times \mbf{v} \right)^\eqm, \qquad \left[ \mbf{u}^\eqp, \mbf{v}^\eqp \right] \equiv \mbf{u}^\eqp \mbf{v}^\eqp - \mbf{v}^\eqp \mbf{u}^\eqp \equiv \left( \mbf{u}^\times \mbf{v} \right)^\eqp \\
\underbrace{\bigl[ \mbf{u}^\eqm, \bigl[ \mbf{u}^\eqm, \ldots \bigl[ \mbf{u}^\eqm,}_{n} \mbf{v}^\eqm\bigr] \ldots \bigr] \bigr] \equiv \left( \left( \mbf{u}^\times \right)^n \mbf{v} \right)^\eqm, \qquad \underbrace{\bigl[ \mbf{u}^\eqp, \bigl[ \mbf{u}^\eqp, \ldots \bigl[ \mbf{u}^\eqp,}_{n} \mbf{v}^\eqp\bigr] \ldots \bigr] \bigr] \equiv \left( \left( \mbf{u}^\times \right)^n \mbf{v} \right)^\eqp \\
\left[ \mbf{u}^\eqm, \mbf{u}^\eqp \right] \equiv \mbf{0} \\
\mbf{y}^\qm = \bbm \mbs{\epsilon} \\ \eta \ebm^\qm := \bbm \eta \mbf{1}  - \mbs{\epsilon}^\times & \mbs{\epsilon} \\ -\mbs{\epsilon}^T & \eta \ebm, \qquad \mbf{y}^\qp = \bbm \mbs{\epsilon} \\ \eta \ebm^\qp := \bbm \eta \mbf{1}  + \mbs{\epsilon}^\times & \mbs{\epsilon} \\ -\mbs{\epsilon}^T & \eta \ebm \\
\mbf{y}^{-1} = \bbm \mbs{\epsilon} \\ \eta \ebm^{-1} := \bbm -\mbs{\epsilon} \\ \eta \ebm \\
(\alpha \mbf{y} + \beta \mbf{z})^\qm \equiv \alpha \mbf{y}^\qm + \beta \mbf{z}^\qm, \qquad (\alpha \mbf{y} + \beta \mbf{z})^\qp \equiv \alpha \mbf{y}^\qp + \beta \mbf{z}^\qp \\
\left( \mbf{y}^\qm \right)^T \equiv \left( \mbf{y}^\qm \right)^{-1} \equiv \left( \mbf{y}^{-1} \right)^\qm, \qquad \left( \mbf{y}^\qp \right)^T \equiv \left( \mbf{y}^\qp \right)^{-1} \equiv \left( \mbf{y}^{-1} \right)^\qp \\
\left( \mbf{y}^\qm \mbf{z} \right)^{-1} \equiv \mbf{z}^{-1^\qm}\mbf{y}^{-1}, \qquad \left( \mbf{y}^\qp \mbf{z} \right)^{-1} \equiv \mbf{z}^{-1^\qp}\mbf{y}^{-1} \\
\left( \mbf{y}^\qm \mbf{z} \right)^\qm \equiv \mbf{y}^\qm \mbf{z}^\qm,  \qquad \left( \mbf{y}^\qp \mbf{z} \right)^\qp \equiv \mbf{y}^\qp \mbf{z}^\qp \\
\mbf{y}^\qm \mbf{z} \equiv \mbf{z}^\qp \mbf{y}, \qquad \mbf{y}^\qm \mbf{z}^\qp \equiv \mbf{z}^\qp \mbf{y}^\qm \\
\mbs{\iota} := \bbm \mbf{0} \\ 1 \ebm, \qquad \mbs{\iota}^\qm \equiv \mbs{\iota}^\qp \equiv \mbf{1} \\
\mbf{y}^\qm \mbf{y}^{-1} \equiv \mbf{y}^\qp \mbf{y}^{-1} \equiv (\mbf{y}^T \mbf{y}) \, \mbs{\iota} \\
\mbf{q} := \bbm \sin \frac{\phi}{2} \mbf{a} \\ \cos\frac{\phi}{2} \ebm = \bbm \mbs{\epsilon} \\ \eta \ebm, \quad \mbf{q}^T \mbf{q} \equiv\mbs{\epsilon}^T\mbs{\epsilon} + \eta^2 \equiv 1 \\ 
\mbf{C} \equiv \left(\eta^2 - \mbs{\epsilon}^T\mbs{\epsilon} \right)\mbf{1} + 2 \mbs{\epsilon}\mbs{\epsilon}^T -2 \eta \mbs{\epsilon}^\times  \\
\mbf{q}^\qm \equiv \cos\frac{\phi}{2} \mbf{1} - 2\sin \frac{\phi}{2} \mbf{a}^\eqm \equiv e^{-\mbs{\phi}^\eqm} \equiv \mbf{1} - \mbs{\phi}^\eqm + \frac{1}{2}  \mbs{\phi}^\eqm  \mbs{\phi}^\eqm  - \cdots \approx \mbf{1} - \mbs{\phi}^\eqm \equiv \bbm \frac{1}{2} \mbs{\phi} \\ 1 \ebm ^\qm \\
\mbf{q}^\qp \equiv \cos\frac{\phi}{2} \mbf{1} - 2\sin \frac{\phi}{2} \mbf{a}^\eqp \equiv e^{-\mbs{\phi}^\eqp} \equiv \mbf{1} - \mbs{\phi}^\eqp + \frac{1}{2}  \mbs{\phi}^\eqp  \mbs{\phi}^\eqp  - \cdots \approx \mbf{1} - \mbs{\phi}^\eqp \equiv \bbm \frac{1}{2} \mbs{\phi} \\ 1 \ebm ^\qp \\
\mbf{q}^\qm \mbf{q}^{-1^\qp} \equiv e^{-\mbs{\phi}^\eqm} e^{\mbs{\phi}^\eqp} \equiv e^{-\mbs{\phi}^\eqm + \mbs{\phi}^\eqp} \equiv e^{- \bbm \mbs{\phi}^\times & \mbf{0} \\ \mbf{0}^T & 0 \ebm} \equiv \bbm e^{-\mbs{\phi}^\times} & \mbf{0} \\ \mbf{0}^T & 1 \ebm \equiv \bbm \mbf{C} & \mbf{0} \\ \mbf{0}^T & 1 \ebm \\
\mbf{q}^\qp \mbf{u}^\eqm \equiv \mbf{u}^\eqm \mbf{q}^\qp, \qquad \mbf{q}^\qm \mbf{u}^\eqp \equiv \mbf{u}^\eqp \mbf{q}^\qm \\
\mbf{q}^\qm \mbf{u}^\eqm \mbf{q}^{-1^\qm} \equiv \left( \mbf{C} \mbf{u} \right)^\eqm, \qquad \mbf{q}^\qm e^{\mbf{u}^\eqm} \mbf{q}^{-1^\qm} \equiv e^{\left( \mbf{C} \mbf{u} \right)^\eqm} \\ 
\mbf{q}^\qp \mbf{u}^\eqp \mbf{q}^{-1^\qp} \equiv \left( \mbf{C} \mbf{u} \right)^\eqp, \qquad \mbf{q}^\qp e^{\mbf{u}^\eqp} \mbf{q}^{-1^\qp} \equiv e^{\left( \mbf{C} \mbf{u} \right)^\eqp}
\end{gather*}


\subsection{{\em SE(3)} Notation}

\noindent
The following definitions, identities, and approximations are useful for {\em SE(3)}.  Much of the $4 \times 4$ notation can be found in \citet{furgale_phd11} and some of the $6 \times 6$ notation can be found in \citet{deleuterio85}, \citet{deleuterio92}.
\begin{gather*}
\mbf{w}^\eff = \bbm \mbf{u} \\ \mbf{v} \ebm^\eff := \bbm \mbf{v}^\times & - \mbf{u} \\ \mbf{0}^T & 0 \ebm, \qquad \mbf{w}^\ess = \bbm \mbf{u} \\ \mbf{v} \ebm^\ess := \bbm \mbf{v}^\times & \mbf{u}^\times \\ \mbf{0} & \mbf{v}^\times \ebm \\ 
\left( \alpha \mbf{w} + \beta \mbf{x} \right)^\eff \equiv \alpha \mbf{w}^\eff + \beta \mbf{x}^\eff, \qquad\left( \alpha \mbf{w} + \beta \mbf{x} \right)^\ess \equiv \alpha \mbf{w}^\ess + \beta \mbf{x}^\ess \\
\mbf{w}^\ess \mbf{x} \equiv - \mbf{x}^\ess \mbf{w}, \qquad \mbf{w}^\ess \mbf{w} \equiv \mbf{0} \\
\left[ \mbf{w}^\eff,  \mbf{x}^\eff \right] \equiv  \mbf{w}^\eff  \mbf{x}^\eff -   \mbf{x}^\eff \mbf{w}^\eff \equiv \left( \mbf{w}^\ess  \mbf{x} \right)^\eff, \qquad \underbrace{\bigl[ \mbf{w}^\eff, \bigl[ \mbf{w}^\eff, \ldots \bigl[ \mbf{w}^\eff,}_{n} \mbf{x}^\eff \bigr] \ldots \bigr] \bigr] \equiv \left( \left( \mbf{w}^\ess \right)^n \mbf{x} \right)^\eff \\
\left[ \mbf{w}^\ess,  \mbf{x}^\ess \right] \equiv  \mbf{w}^\ess  \mbf{x}^\ess -   \mbf{x}^\ess \mbf{w}^\ess \equiv \left( \mbf{w}^\ess  \mbf{x} \right)^\ess, \qquad \underbrace{\bigl[ \mbf{w}^\ess, \bigl[ \mbf{w}^\ess, \ldots \bigl[ \mbf{w}^\ess,}_{n} \mbf{x}^\ess \bigr] \ldots \bigr] \bigr] \equiv \left( \left( \mbf{w}^\ess \right)^n \mbf{x} \right)^\ess  \\
\mbs{\pi} := \bbm \mbs{\rho} \\ \mbs{\phi} \ebm \\
\mbf{T} := \bbm \mbf{C} & \mbf{r}  \\ \mbf{0}^T & 1 \ebm \equiv \bbm \mbf{C} & \mbf{S} \mbs{\rho} \\ \mbf{0}^T & 1 \ebm \equiv e^{-\mbs{\pi}^\eff} \equiv \mbf{1} - \mbs{\pi}^\eff + \frac{1}{2} \mbs{\pi}^\eff \mbs{\pi}^\eff - \cdots \approx \mbf{1} - \mbs{\pi}^\eff  \\
\mbs{\mathcal{T}} := \mbf{T}^\Tss = \bbm \mbf{C} & \mbf{r}  \\ \mbf{0}^T & 1 \ebm^\Tss := \bbm \mbf{C} & -\mbf{r}^\times \mbf{C} \\ \mbf{0} & \mbf{C} \ebm \equiv \bbm \mbf{C} & -\left( \mbf{S} \mbs{\rho} \right)^\times \mbf{C} \\ \mbf{0} & \mbf{C} \ebm \equiv e^{-\mbs{\pi}^\ess} \equiv \mbf{1} - \mbs{\pi}^\ess + \frac{1}{2} \mbs{\pi}^\ess \mbs{\pi}^\ess - \cdots \approx \mbf{1} - \mbs{\pi}^\ess \\
\left( \mbf{T}_1 \mbf{T}_2 \right)^\Tss = \mbf{T}_1^\Tss \mbf{T}_2^\Tss \\
\mbox{tr}(\mbf{T}) \equiv 2 \cos\phi + 2, \qquad \mbox{det} (\mbf{T}) \equiv 1 \\
\mbf{T}^{-1} \equiv \bbm \mbf{C}^T & -\mbf{C}^T \mbf{r} \\ \mbf{0}^T & 1 \ebm \approx \mbf{1} + \mbs{\pi}^\eff \\ 
\mbs{\mathcal{T}}^{-1} := \left( \mbf{T}^{-1} \right)^\Tss \equiv  \bbm \mbf{C}^T & \mbf{C}^T \mbf{r}^\times \\ \mbf{0} & \mbf{C}^T \ebm \approx \mbf{1} + \mbs{\pi}^\ess \\ 
\left(e^{-\mbs{\pi}^\eff}\right)^\Tss \equiv e^{-\mbs{\pi}^\ess} \\
\left( \mbs{\mathcal{T}} \mbf{w} \right)^\eff \equiv \mbf{T} \mbf{w}^\eff \mbf{T}^{-1}, \qquad e^{\left(\mbs{\mathcal{T}}\mbf{w}\right)^\eff}  \equiv \mbf{T} e^{\mbf{w}^\eff} \mbf{T}^{-1} \\
\left( \mbs{\mathcal{T}} \mbf{w} \right)^\ess \equiv \mbs{\mathcal{T}} \mbf{w}^\ess \mbs{\mathcal{T}}^{-1}, \qquad  e^{\left(\mbs{\mathcal{T}}\mbf{w}\right)^\ess} \equiv \mbs{\mathcal{T}} e^{\mbf{w}^\ess} \mbs{\mathcal{T}}^{-1} \\
\left( \mbf{w}^\eff \mbf{T} \right)^\Tss \equiv \mbf{w}^\ess \mbs{\mathcal{T}} \\
\mbs{\mathcal{S}} := \int_0^1 \mbs{\mathcal{T}}^{\alpha} \, d\alpha \equiv \sum_{n=0}^\infty (-1)^n \frac{1}{(n+1)!} \left( \mbs{\pi}^\ess \right)^n \equiv \bbm \mbf{S} & \mbf{Q} \\ \mbf{0} & \mbf{S} \ebm \\
\mbs{\mathcal{S}}^{-1} \equiv \sum_{n=0}^\infty (-1)^n \frac{B_n}{n!} \left( \mbs{\pi}^\ess \right)^n \equiv \bbm \mbf{S}^{-1} & -\mbf{S}^{-1}\mbf{Q}\mbf{S}^{-1} \\ \mbf{0} & \mbf{S}^{-1} \ebm 
\end{gather*}
\begin{gather*}
\mbf{Q} := \sum_{n=0}^\infty \sum_{m=0}^\infty \frac{(-1)^{n+m+1}}{(n+m+2)!} \,\left(\mbs{\phi}^\times\right)^n \mbs{\rho}^\times \left(\mbs{\phi}^\times \right)^m \\
%-\frac{1}{2!} \mbs{\rho}^\times + \frac{1}{3!} \left( \mbs{\phi}^\times\mbs{\rho}^\times + \mbs{\rho}^\times \mbs{\phi}^\times \right) - \frac{1}{4!}\left(  \mbs{\phi}^\times\mbs{\phi}^\times\mbs{\rho}^\times + \mbs{\phi}^\times\mbs{\rho}^\times\mbs{\phi}^\times + \mbs{\rho}^\times\mbs{\phi}^\times\mbs{\phi}^\times\right) + \cdots \\
\quad\, \equiv -\frac{1}{2} \mbs{\rho}^\times + \frac{\phi-\sin\phi}{\phi^3} \left(  \mbs{\phi}^\times \mbs{\rho}^\times + \mbs{\rho}^\times \mbs{\phi}^\times - \mbs{\phi}^\times \mbs{\rho}^\times \mbs{\phi}^\times \right) + \frac{1-\frac{\phi^2}{2}-\cos\phi}{\phi^4} \left( \mbs{\phi}^\times \mbs{\phi}^\times \mbs{\rho}^\times + \mbs{\rho}^\times \mbs{\phi}^\times \mbs{\phi}^\times -3 \mbs{\phi}^\times \mbs{\rho}^\times \mbs{\phi}^\times \right) \\
\qquad\qquad\qquad - \frac{1}{2} \left( \frac{1-\frac{\phi^2}{2}-\cos\phi}{\phi^4} - 3 \frac{\phi - \sin\phi - \frac{\phi^3}{6}}{\phi^5}\right) \left( \mbs{\phi}^\times \mbs{\rho}^\times \mbs{\phi}^\times\mbs{\phi}^\times + \mbs{\phi}^\times\mbs{\phi}^\times \mbs{\rho}^\times \mbs{\phi}^\times \right) \\
e^{-\left(\mbf{w} + \mbs{\pi}\right)^\eff} \approx e^{-(\mbs{\mathcal{S}} \mbf{w})^\eff} \mbf{T}, \qquad \mbox{(correct to first order in $\mbf{w}$)} \\
e^{-\left(\mbf{w} + \mbs{\pi}\right)^\ess} \approx e^{-(\mbs{\mathcal{S}} \mbf{w})^\ess} \mbs{\mathcal{T}}, \qquad \mbox{(correct to first order in $\mbf{w}$)} \\
\mbs{\mathcal{T}} \equiv \mbf{1} - \mbs{\pi}^\ess \mbs{\mathcal{S}} \\
\frac{\partial \left( \mbf{T} \mbf{p} \right) }{\partial \mbs{\pi}} =  \left( \mbf{T} \mbf{p} \right)^\pfs \mbs{\mathcal{S}} \\
\frac{\partial \left( \mbs{\mathcal{T}} \mbf{w} \right) }{\partial \mbs{\pi}} =  \left( \mbs{\mathcal{T}} \mbf{w} \right)^\ess \mbs{\mathcal{S}} \\
\mbs{\mathcal{S}}(\mbs{\pi}) \equiv \mbs{\mathcal{T}}(\mbs{\pi}) \, \mbs{\mathcal{S}}(-\mbs{\pi})
\end{gather*}


\subsection{Homogenous Point Notation}

The following definitions, identities, and approximations are useful for representing three-dimensional points in homogeneous coordinates.  Some of this notation can be found in \citet{furgale_phd11}.
\begin{gather*}
\mbf{y} := \bbm \mbs{\epsilon} \\ \eta \ebm \\
\mbf{y}^\pfs := \bbm \eta \mbf{1} & \mbs{\epsilon}^\times \\ \mbf{0}^T & \mbf{0}^T \ebm, \qquad \left( \mbf{T} \mbf{y} \right)^\pfs \equiv \mbf{T} \, \mbf{y}^\pfs \, \mbf{T}^{-\Tss} \\
\mbf{w}^\eff \mbf{y} \equiv -\mbf{y}^\pfs \mbf{w} \\
\mbf{y}^\psf := \bbm \mbf{0} & \mbs{\epsilon}  \\  \mbs{\epsilon}^\times & \mbf{0} \ebm \\
\mbf{y}^T \mbf{w}^\eff \equiv -\mbf{w}^T \mbf{y}^\psf \\
\mbf{y}^\pftm := \frac{1}{2} \bbm \eta \mbf{1} + \mbs{\epsilon}^\times \\ -\mbs{\epsilon}^T \ebm \equiv  \mbf{y}^\qp \mbf{V}, \qquad \mbf{y}^\pftp := \frac{1}{2} \bbm \eta \mbf{1} - \mbs{\epsilon}^\times \\ -\mbs{\epsilon}^T \ebm \equiv \mbf{y}^\qm \mbf{V}, \qquad \mbf{V} := \frac{1}{2} \bbm 1 & 0 & 0 \\ 0 & 1 & 0 \\ 0 & 0 & 1 \\ 0 & 0 & 0 \ebm \\
\mbf{u}^\eqm \mbf{y} \equiv -\mbf{y}^\pftm \mbf{u}, \qquad \mbf{u}^\eqp \mbf{y} \equiv -\mbf{y}^\pftp \mbf{u} \\
\mbf{y}^T \mbf{u}^\eqm \equiv \mbf{u}^T \mbf{y}^{\pftm^T}, \qquad \mbf{y}^T \mbf{u}^\eqp \equiv \mbf{u}^T \mbf{y}^{\pftp^T}
\end{gather*}

